Assessing Coarse-to-Fine Deep Learning Models for Optic Disc and Cup Segmentation in Fundus Images

Automated optic disc (OD) and optic cup (OC) segmentation in fundus images is relevant to efficiently measure the vertical cup-to-disc ratio (vCDR), a biomarker commonly used in ophthalmology to determine the degree of glaucomatous optic neuropathy. In general this is solved using coarse-to-fine deep learning algorithms in which a first stage approximates the OD and a second one uses a crop of this area to predict OD/OC masks. While this approach is widely applied in the literature, there are no studies analyzing its real contribution to the results. In this paper we present a comprehensive analysis of different coarse-to-fine designs for OD/OC segmentation using 5 public databases, both from a standard segmentation perspective and for estimating the vCDR for glaucoma assessment. Our analysis shows that these algorithms not necessarily outperfom standard multi-class single-stage models, especially when these are learned from sufficiently large and diverse training sets. Furthermore, we noticed that the coarse stage achieves better OD segmentation results than the fine one, and that providing OD supervision to the second stage is essential to ensure accurate OC masks. Moreover, both the single-stage and two-stage models trained on a multi-dataset setting showed results in pair or even better than other state-of-the-art alternatives, while ranking first in REFUGE for OD/OC segmentation. Finally, we evaluated the models for vCDR prediction in comparison with six ophthalmologists on a subset of AIROGS images, to understand them in the context of inter-observer variability. We noticed that vCDR estimates recovered both from single-stage and coarse-to-fine models can obtain good glaucoma detection results even when they are not highly correlated with manual measurements from experts.

==> old_code.tex <==

Begin the Introduction below the Keywords. The manuscript should not have headers, footers, or page numbers. It should be in a one-column format. References are often noted in the text and cited at the end of the paper.

\begin{table}[ht]
\caption{Fonts sizes to be used for various parts of the manuscript.  Table captions should be centered above the table.  When the caption is too long to fit on one line, it should be justified to the right and left margins of the body of the text.} 
\label{tab:fonts}
\begin{center}       
\begin{tabular}{|l|l|} %% this creates two columns
%% |l|l| to left justify each column entry
%% |c|c| to center each column entry
%% use of \rule[]{}{} below opens up each row
\hline
\rule[-1ex]{0pt}{3.5ex}  Article title & 16 pt., bold, centered  \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Author names and affiliations & 12 pt., normal, centered   \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Keywords & 10 pt., normal, left justified   \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Abstract Title & 11 pt., bold, centered   \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Abstract body text & 10 pt., normal, justified   \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Section heading & 11 pt., bold, centered (all caps)  \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Subsection heading & 11 pt., bold, left justified  \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Sub-subsection heading & 10 pt., bold, left justified  \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Normal text & 10 pt., normal, justified  \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Figure and table captions & \, 9 pt., normal \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Footnote & \, 9 pt., normal \\
\hline 
\rule[-1ex]{0pt}{3.5ex}  Reference Heading & 11 pt., bold, centered   \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Reference Listing & 10 pt., normal, justified   \\
\hline
\end{tabular}
\end{center}
\end{table} 

\begin{table}[ht]
\caption{Margins and print area specifications.} 
\label{tab:Paper Margins}
\begin{center}       
\begin{tabular}{|l|l|l|} 
\hline
\rule[-1ex]{0pt}{3.5ex}  Margin & A4 & Letter  \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Top margin & 2.54 cm & 1.0 in.   \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Bottom margin & 4.94 cm & 1.25 in.  \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Left, right margin & 1.925 cm & .875 in.  \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Printable area & 17.15 x 22.23 cm & 6.75 x 8.75 in.  \\
\hline 
\end{tabular}
\end{center}
\end{table}

LaTeX margins are related to the document's paper size. The paper size is by default set to USA letter paper. To format a document for A4 paper, the first line of this LaTeX source file should be changed to \verb|\documentclass[a4paper]{spie}|.   

Authors are encouraged to follow the principles of sound technical writing, as described in Refs.~\citenum{Alred03} and \citenum{Perelman97}, for example.  Many aspects of technical writing are addressed in the {\em AIP Style Manual}, published by the American Institute of Physics.  It is available on line at \url{https://publishing.aip.org/authors}. A spelling checker is helpful for finding misspelled words. 

An author may use this LaTeX source file as a template by substituting his/her own text in each field.  This document is not meant to be a complete guide on how to use LaTeX.  For that, please see the list of references at \url{http://latex-project.org/guides/} and for an online introduction to LaTeX please see \citenum{Lees-Miller-LaTeX-course-1}. 

\section{FORMATTING OF MANUSCRIPT COMPONENTS}

This section describes the normal structure of a manuscript and how each part should be handled.  The appropriate vertical spacing between various parts of this document is achieved in LaTeX through the proper use of defined constructs, such as \verb|\section{}|.  In LaTeX, paragraphs are separated by blank lines in the source file. 

At times it may be desired, for formatting reasons, to break a line without starting a new paragraph.  This situation may occur, for example, when formatting the article title, author information, or section headings.  Line breaks are inserted in LaTeX by entering \verb|\\| or \verb|\linebreak| in the LaTeX source file at the desired location.  

\subsection{Title and Author Information}
\label{sec:title}

The article title appears centered at the top of the first page.  The title font is 16 point, bold.  The rules for capitalizing the title are the same as for sentences; only the first word, proper nouns, and acronyms should be capitalized.  Avoid using acronyms in the title.  Keep in mind that people outside your area of expertise might read your article. At the first occurrence of an acronym, spell it out, followed by the acronym in parentheses, e.g., noise power spectrum (NPS). 

The author list is in 12-pt. regular, centered. Omit titles and degrees such as Dr., Prof., Ph.D., etc. The list of affiliations follows the author list. Each author's affiliation should be clearly noted. Superscripts may be used to identify the correspondence between the authors and their respective affiliations.  Further author information, such as e-mail address, complete postal address, and web-site location, may be provided in a footnote by using \verb|\authorinfo{}|, as demonstrated above.

\subsection{Abstract and Keywords}
The title and author information is immediately followed by the Abstract. The Abstract should concisely summarize the key findings of the paper.  It should consist of a single paragraph containing no more than 250 words.  The Abstract does not have a section number.  A list of up to eight keywords should immediately follow the Abstract after a blank line.  These keywords will be included in a searchable database at SPIE.

\subsection{Body of Paper}
The body of the paper consists of numbered sections that present the main findings.  These sections should be organized to best present the material.  See Sec.~\ref{sec:sections} for formatting instructions.

\subsection{Appendices}
Auxiliary material that is best left out of the main body of the paper, for example, derivations of equations, proofs of theorems, and details of algorithms, may be included in appendices.  Appendices are enumerated with uppercase Latin letters in alphabetic order, and appear just before the Acknowledgments and References. Appendix~\ref{sec:misc} contains more about formatting equations and theorems.

\subsection{Acknowledgments}
In the Acknowledgments section, appearing just before the References, the authors may credit others for their guidance or help.  Also, funding sources may be stated.  The Acknowledgments section does not have a section number.

\subsection{References}
SPIE is able to display the references section of your paper in the SPIE Digital Library, complete with links to referenced journal articles, proceedings papers, and books, when available. This added feature will bring more readers to your paper and improve the usefulness of the SPIE Digital Library for all researchers. The References section does not have a section number.  The references are numbered in the order in which they are cited.  Examples of the format to be followed are given at the end of this document.  

The reference list at the end of this document is created using BibTeX, which looks through the file {\ttfamily report.bib} for the entries cited in the LaTeX source file.  The format of the reference list is determined by the bibliography style file {\ttfamily spiebib.bst}, as specified in the \verb|\bibliographystyle{spiebib}| command.  Alternatively, the references may be directly formatted in the LaTeX source file.

For books\cite{Lamport94,Alred03,Goossens97}, the listing includes the list of authors, book title, publisher, city, page or chapter numbers, and year of publication.  A reference to a journal article\cite{Metropolis53} includes the author list, title of the article (in quotes), journal name (in italics, properly abbreviated), volume number (in bold), inclusive page numbers, and year.  By convention\cite{Lamport94}, article titles are capitalized as described in Sec.~\ref{sec:title}.  A reference to a proceedings paper or a chapter in an edited book\cite{Gull89a} includes the author list, title of the article (in quotes), volume or series title (in italics), volume number (in bold), if applicable, inclusive page numbers, publisher, city, and year.  References to an article in the SPIE Proceedings may include the conference name (in italics), as shown in Ref.~\citenum{Hanson93c}. For websites\cite{Lees-Miller-LaTeX-course-1} the listing includes the list of authors, title of the article (in quotes), website name, article date, website address either enclosed in chevron symbols ('\(<\)' and '\(>\)'),  underlined or linked, and the date the website was accessed. 

If you use this formatting, your references will link your manuscript to other research papers that are in the CrossRef system. Exact punctuation is required for the automated linking to be successful. 

Citations to the references are made using superscript numerals, as demonstrated in the above paragraph.  One may also directly refer to a reference within the text, e.g., ``as shown in Ref.~\citenum{Metropolis53} ...''

\subsection{Footnotes}
Footnotes\footnote{Footnotes are indicated as superscript symbols to avoid confusion with citations.} may be used to provide auxiliary information that doesn't need to appear in the text, e.g., to explain measurement units.  They should be used sparingly, however.  

Only nine footnote symbols are available in LaTeX. If you have more than nine footnotes, you will need to restart the sequence using the command  \verb|\footnote[1]{Your footnote text goes here.}|. If you don't, LaTeX will provide the error message {\ttfamily Counter too large.}, followed by the offending footnote command.

\section{SECTION FORMATTING}
\label{sec:sections}

Section headings are centered and formatted completely in uppercase 11-point bold font.  Sections should be numbered sequentially, starting with the first section after the Abstract.  The heading starts with the section number, followed by a period.  In LaTeX, a new section is created with the \verb|\section{}| command, which automatically numbers the sections.

Paragraphs that immediately follow a section heading are leading paragraphs and should not be indented, according to standard publishing style\cite{Lamport94}.  The same goes for leading paragraphs of subsections and sub-subsections.  Subsequent paragraphs are standard paragraphs, with 14-pt.\ (5 mm) indentation.  An extra half-line space should be inserted between paragraphs.  In LaTeX, this spacing is specified by the parameter \verb|\parskip|, which is set in {\ttfamily spie.cls}.  Indentation of the first line of a paragraph may be avoided by starting it with \verb|\noindent|.
 
\subsection{Subsection Attributes}

The subsection heading is left justified and set in 11-point, bold font.  Capitalization rules are the same as those for book titles.  The first word of a subsection heading is capitalized.  The remaining words are also capitalized, except for minor words with fewer than four letters, such as articles (a, an, and the), short prepositions (of, at, by, for, in, etc.), and short conjunctions (and, or, as, but, etc.).  Subsection numbers consist of the section number, followed by a period, and the subsection number within that section.  

\subsubsection{Sub-subsection attributes}
The sub-subsection heading is left justified and its font is 10 point, bold.  Capitalize as for sentences.  The first word of a sub-subsection heading is capitalized.  The rest of the heading is not capitalized, except for acronyms and proper names.  

\section{FIGURES AND TABLES}

Figures are numbered in the order of their first citation.  They should appear in numerical order and on or after the same page as their first reference in the text.  Alternatively, all figures may be placed at the end of the manuscript, that is, after the Reference section.  It is preferable to have figures appear at the top or bottom of the page.  Figures, along with their captions, should be separated from the main text by at least 0.2 in.\ or 5 mm.  

Figure captions are centered below the figure or graph.  Figure captions start with the figure number in 9-point bold font, followed by a period; the text is in 9-point normal font; for example, ``{\footnotesize{Figure 3.}  Original image...}''.  See Fig.~\ref{fig:example} for an example of a figure caption.  When the caption is too long to fit on one line, it should be justified to the right and left margins of the body of the text.  

Tables are handled identically to figures, except that their captions appear above the table. 

% Note: If compiling with LaTeX+dvipdf, please ensure images generated from 
% other software packages have their bounding boxes set correctly.
   \begin{figure} [ht]
   \begin{center}
   \begin{tabular}{c} %% tabular useful for creating an array of images 
   \includegraphics[height=5cm]{mcr3b.eps}
   \end{tabular}
   \end{center}
   \caption[example] 
%>>>> use \label inside caption to get Fig. number with \ref{}
   { \label{fig:example} 
Figure captions are used to describe the figure and help the reader understand it's significance.  The caption should be centered underneath the figure and set in 9-point font.  It is preferable for figures and tables to be placed at the top or bottom of the page. LaTeX tends to adhere to this standard.}
   \end{figure} 

\section{MULTIMEDIA FIGURES - VIDEO AND AUDIO FILES}

Video and audio files can be included for publication. See Tab.~\ref{tab:Multimedia-Specifications} for the specifications for the mulitimedia files. Use a screenshot or another .jpg illustration for placement in the text. Use the file name to begin the caption. The text of the caption must end with the text ``http://dx.doi.org/doi.number.goes.here'' which tells the SPIE editor where to insert the hyperlink in the digital version of the manuscript. 

Here is a sample illustration and caption for a multimedia file:

   \begin{figure} [ht]
   \begin{center}
   \begin{tabular}{c} 
   \includegraphics[height=5cm]{MultimediaFigure.jpg}
	\end{tabular}
	\end{center}
   \caption[example] 
   { \label{fig:video-example} 
A label of “Video/Audio 1, 2, …” should appear at the beginning of the caption to indicate to which multimedia file it is linked . Include this text at the end of the caption: \url{http://dx.doi.org/doi.number.goes.here}}
   \end{figure} 
   
   \begin{table}[ht]
\caption{Information on video and audio files that must accompany a manuscript submission.} 
\label{tab:Multimedia-Specifications}
\begin{center}       
\begin{tabular}{|l|l|l|}
\hline
\rule[-1ex]{0pt}{3.5ex}  Item & Video & Audio  \\
\hline
\rule[-1ex]{0pt}{3.5ex}  File name & Video1, video2... & Audio1, audio2...   \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Number of files & 0-10 & 0-10  \\
\hline
\rule[-1ex]{0pt}{3.5ex}  Size of each file & 5 MB & 5 MB  \\
\hline
\rule[-1ex]{0pt}{3.5ex}  File types accepted & .mpeg, .mov (Quicktime), .wmv (Windows Media Player) & .wav, .mp3  \\
\hline 
\end{tabular}
\end{center}
\end{table}

\appendix    %>>>> this command starts appendixes

\section{MISCELLANEOUS FORMATTING DETAILS}
\label{sec:misc}

It is often useful to refer back (or forward) to other sections in the article.  Such references are made by section number.  When a section reference starts a sentence, Section is spelled out; otherwise use its abbreviation, for example, ``In Sec.~2 we showed...'' or ``Section~2.1 contained a description...''.  References to figures, tables, and theorems are handled the same way.

\subsection{Formatting Equations}
Equations may appear in line with the text, if they are simple, short, and not of major importance; e.g., $\beta = b/r$.  Important equations appear on their own line.  Such equations are centered.  For example, ``The expression for the field of view is
\begin{equation}
\label{eq:fov}
2 a = \frac{(b + 1)}{3c} \, ,
\end{equation}
where $a$ is the ...'' Principal equations are numbered, with the equation number placed within parentheses and right justified.  

Equations are considered to be part of a sentence and should be punctuated accordingly. In the above example, a comma follows the equation because the next line is a subordinate clause.  If the equation ends the sentence, a period should follow the equation.  The line following an equation should not be indented unless it is meant to start a new paragraph.  Indentation after an equation is avoided in LaTeX by not leaving a blank line between the equation and the subsequent text.

References to equations include the equation number in parentheses, for example, ``Equation~(\ref{eq:fov}) shows ...'' or ``Combining Eqs.~(2) and (3), we obtain...''  Using a tilde in the LaTeX source file between two characters avoids unwanted line breaks.

\subsection{Formatting Theorems}

To include theorems in a formal way, the theorem identification should appear in a 10-point, bold font, left justified and followed by a period.  The text of the theorem continues on the same line in normal, 10-point font.  For example, 

\noindent\textbf{Theorem 1.} For any unbiased estimator...

Formal statements of lemmas and algorithms receive a similar treatment.

\acknowledgments % equivalent to \section*{ACKNOWLEDGMENTS}       
 
This unnumbered section is used to identify those who have aided the authors in understanding or accomplishing the work presented and to acknowledge sources of funding.  


==> old_code_2.tex <==

% \jio{La segmentación automática del disco óptico (OD) y la copa óptica (OC) en imágenes de fondo de ojo es útil para mejorar el cálculo de la relación vertical copa disco, un biomarcador utilizado comunmente para determinar el grado de neuropatía óptica glaucomatosa.
% %
% En general se lo resuelve utilizando coarse-to-fine deep learning algorithms, en los cuales una primera etapa se encarga de aproximar el area del disco, y la segunda toma esta región como entrada para segmentar mejor el disco y la copa.
% %
% A pesar de la popularidad de estos enfoques, no existen trabajos que estudien empiricamente la contribución de este tipo de arquitecturas sobre los resultados.
% %
% En este trabajo presentamos un estudio detallado de diferentes versiones de modelos coarse-to-fine para la segmentación de disco y copa óptica.
% %
% Además de analizar la precision de las segmentaciones, realizamos una evaluación de su efectividad para la estimación del vCDR comparando las predicciones obtenidas con las mediciones realizadas por seis expertos sobre un banco de datos que construimos especialmente para este analisis.
% %
% Nuestro analisis mostro que estos algoritmos no necesariamente superan los resultados de versiones clásicas basadas en una etapa, sobre todo cuando los conjuntos de entrenamiento cuentan con un número importante de imágenes.
% %
% Observamos también que la etapa coarse suele obtener mejores resultados para segmentación de disco que la etapa fine, pero que supervisar a la etapa fine con información del disco es necesario para asegurar buenos resultados para OC segmentation.
% %
% Además, comprobamos que aumentar la entrada de la etapa fine con la salida de la etapa coarse permite en algunos casos mejorar los resultados para segmentación de copa.
% %

%Glaucoma is currently the second leading cause of blindness in the world\cite{orlando2020refuge,kovalyk2022papila}. It is estimated that by 2040, 111.8 million people between the ages of 40 and 80 will suffer from this disease. Glaucoma is a silent disease that can lead to irreversible blindness if not detected and treated in time. The main characteristic of this disease is an unstable or sustained increase in intra-ocular pressure that the eye cannot withstand, resulting in damage to the optic nerve and consequent loss of vision. Currently, there is no cure for glaucoma, but with early detection, it can be controlled before vision loss occurs. Moreover, because there are no alarming symptoms of the disease, half of the people with glaucoma do not know they are affected; in some developing countries, 90\% of glaucoma sufferers remain undetected\cite{glaucoma}. 

%fondus imaging is limited for diseases like glaucoma because it is a projective image, i.e. a 2D image, and the depth of the eyecup is lost. 

%Nevertheless, studies have observed that subjects with glaucoma have a reduced vertical cup-to-disc ratio (vCDR), which allows evaluating the level of ocular disc crushing due to ocular pressure. 

%Therefore, segmentation of the optic disc and cup becomes crucial for the early detection of glaucoma. Nevertheless, performing manual segmentation of the ocular disc and cup is time-consuming and tedious for experts. In turn, segmentation is subject to high inter-observer and intra-observer variability. Because of this, several approaches have focused on automatically segmenting the optic disc and cup. \cite{li2021applications,orlando2020refuge}.

%The literature shows OD/OC segmentation as a multi-class segmentation problem. A solution to it could be approximated using a multi-class fully convolutional neural network that will take the image as input and predict score maps for the OD and the OC. The model is trained using mini-batches of a fixed resolution. As fundus images are too big, needed to be downsized for creating the mini-batches. The literature hypothesises that this process affects the edges of the target structures and might reduce the quality of the results.
%So, alternatively, authors use two-stage models for OD/OC segmentation are in general based on twin architectures as those shown in Figure~\ref{fig:schematic}. The first stage takes the entire fundus picture as input and predicts a pixel-wise probability map with the segmentation of the OD. This output is then up-sampled to match the resolution of the original image and used for cropping the area around the optic nerve head. Then, this cropped image is downsized to the exact resolution used for training the first stage and used as input for the second one, which simultaneously segments the OD/OC. The hypothesis behind this decision is that feeding the second stage with an image in which the optic nerve head appears approximately at the exact resolution as the original image will result in much better segmentations. 

%Some authors instantiated the two stages using architectures such as U-Nerts \cite{wang2019patch} for both stages. Others propose a network for the first stage and an architecture U-net for the second stage  \cite{shah2019dynamic}. Alternatively, it has also been explored to use an objects detector in the first stage and then a segmentation model in the second one \cite{liu2021joint}. Others two-step models can be seen in several papers submitted to REFUGE\cite{orlando2020refuge} and REFUGE2\cite{fang2022refuge2} challenges.

%However, to the best of our knowledge, this design decision is usually reported in the prior art without supporting it with an in-depth ablation analysis of its contribution to the final results. This renders models that might be accurate in some datasets or under specific settings without enough guarantees to perform equally in other more general clinical scenarios

%We propose performing an ablation study to test whether a two-stage model achieves improved disc and cup segmentation. Multiple alternative two-stage approaches were tested and compared against a more straightforward one-stage model. In turn, multiple public datasets were used for this study, allowing us to analyse how the training dataset can affect the quality of the model. Moreover, allowing for a more robust evaluation of the models. The recently published PAPILA \cite{kovalyk2022papila} was among the datasets used. On the other hand, in addition to evaluating segmentation, the vCDR was calculated from the segmentation to analyse the model's effectiveness for automatic glaucoma recognition. Finally, a dataset of vCDR estimates made by six experts was generated from AIROGS [cita a airogs] images and compared with our predictions to study them concerning inter-observer variability.

%MATERIALS AND METHODS 

% In the literature, it is common to see that segmentation is divided into two stages [CITAS]. In the first stage, the entire image is used, reduced in size, to a model that returns an approximated segmentation of the optical disc. Then, the original image is cropped in the area of interest with the segmentation obtained. Then, the cut image is used in a second model that segments the disc and the ocular cup. In this work, we will name this model as $OD-OD\&OC$. In addition to this model, we will analyze variations of this strategy, especially in the second stage. Also, we will compare the two-stage models against a single-stage model. The models analyzed were the following:

% The purpose of this work is to perform a study on two-stage models and how it contributes to improving the segmentation results of both the optic disc (OD) and the optic cup (OC). To this end, we perform an ablation study in which we will study the models illustrated in Figure \ref{fig:schematic}. On the one hand, we train a single-stage network that predicts OD and OC (SS-Model). Alternatively, three different versions of the two-stage model were proposed, which were:

% \begin{itemize}
%     \item \textbf{TS-MODEL OD - OD\&OC}, which corresponds to the model used in most of the studied articles \cite{wang2019patch,shah2019dynamic,liu2021joint}, in which, in the first stage, the model classifies only the OD. From the resulting segmentation, the original image is cropped in the area of interest. Then, a second model segments OD/OC from the cropped image.
%     \item \textbf{TS-MODEL OD - OC}, an alternative model proposed by us, in which the first stage remains the same as the previous model, but the second stage only segments OC. It allows the entire capacity of the second model to be dedicated explicitly to the optic cup segmentation. However, it does not use any information from the disc for prediction.
%     \item \textbf{TS-MODEL OD $\rightarrow$ OD\&OC}, also corresponds to a proposed modification of the TS-MODEL OD - OD&OC model. The first stage is maintained. However, we send the first stage segmentation to the second stage, in addition to the cropped image. We hypothesise that this auxiliary input could simplify the task to the second stage by providing auto-contextuality\cite{tu2009auto}, allowing better results.

% \end{itemize}

%Nuestro propósito es estudiar si efectivamente utilizar dos etapas contribuye a mejorar los resultados de segmentación de OD/OC. Para ello, planteamos un estudio de ablación en el que estudiamos los modelos ilustrados en la Figura XXXX. Por un lado, entrenamos una red en una sola etapa que predice OD/OC (SS-MODEL). Alternativamente, planteamos tres versiones diferentes del modelo a dos etapas, a saber:
%\begin{itemize}
   % \item \textbf{TS-MODEL OD - OD\&OC}, que corresponde al modelo utilizado en la mayor parte de los trabajos relevados (citas), en donde la primera etapa aproxima el disco y se utiliza como guía para recortar la región del optic nerve head, y luego la segunda predice tanto el OD como el OC de manera multiclase.
  %  \item \textbf{TS-MODEL OD - OC}, que corresponde a un modelo alternativo propuesto por nosotros, donde la segunda etapa predice únicamente la segmentación de la OC. Esto permite que toda la capacidad de la segunda etapa se dedique a obtener esta predicción. No utiliza ningún tipo de información acerca del disco para entrenarse. 
 %   \item \textbf{TS-MODEL OD \rightarrow OD\&OC}, que corresponde a una modificación de TS-UNET OD - OD\&OC en donde la segunda etapa recibe como entrada no solamente el recorte de la imagen en la zona del nervio óptico si no también la segmentación del mismo generada por la primera etapa. Nuestra hipótesis es que esta entrada auxiliar podría simplificar la tarea a la segunda etapa ya que brinda autocontext, permitiéndole obtener mejores resultados. We also assume that the model that sends the first segmentation to the second stage will obtain better results by having information from the previous stage, such as the intermediate segmentation.
%\end{itemize}

%\begin{enumerate}
%    \item TS-UNET $OD-OC$: a model that classifies the optical disc in the first stage and segments the optical cup in the second stage.
%    \item TS-UNET $OD\rightarrow OD\&OC$: A model that classifies the optic disc in the first stage. In the second step, in addition to receiving the cropped image, the model received the segmentation from the first step and then segmented the optic disc and optic cup.
%    \item SS-UNET or $OD\&OC$: a model that segments the optic disc and the optic cup with only one model.
%\end{enumerate}

%We train the SS-MODEL and the first stage of the TS-MODELs similarly. First, we obtain an approximate field of view (FOV) mask using the Hough transform [cita?]. Using this mask over the training and validation data, we crop the images around the FOV. Subsequently, the images and their labels were downsampled to a fixed resolution of 512x512 pixels and standardized using their own mean and deviation.

%We should estimate the centre of the binary segmentation of the disc for this crop. However, this centre was randomly shifted in height and width to give more robustness to potential erroneous predictions produced by the first stage. As a result, the optical disc is not always at the centre of the cropped image. The input then undergoes a resolution change to 512x512 pixels, and the image is standardized with its own mean and standar desviation.

%The second stage of the TS-model was trained separately from the first stage. We use the reference segmentation of the OD to crop the image and its label around the optic nerve head. $Delta$ margins of 10\% of the input width and height were used for cropping images to include part of the structures near the nerve region. We should estimate the centre of the binary segmentation of the disc for this crop. However, this centre was randomly shifted in height and width to give more robustness to potential erroneous predictions produced by the first stage. As a result, the optical disc is not always at the centre of the cropped image. The input then undergoes a resolution change to 512x512 pixels, and the image is standardized with its own mean and standar desviation.

%We used several public datasets for our experiments, as shown in Table \ref{tab:datasets}. This are REFUGE \cite{orlando2020refuge} (1200 images), DRISHTI \cite{sivaswamy2014drishti} (100 images), IDRIDTI \cite{porwal2018indian} (81 images), ORIGA \cite{zhang2010origa} (650 images), RIGA \cite{almazroa2018retinal} (749 images), RIM ONE V3 \cite{fumero2011rim} (159 images) and the newly released PAPILA \cite{kovalyk2022papila} (489 images). All the datasets consist of full fundus images, except for the RIM ONE dataset, which has images cropped in the optic disc area. We also generated a small dataset of 40 images from the AIROGS dataset\cite{aimyshevglaucoma_airogs} to compare us with experts.

%We generated three sets of training data. On the one hand, we train the models using only DRISHTI data. On the other hand, just using REFUGE data. Moreover, we use a multi-dataset which has different datasets together for training. This multi-dataset was divided into training, validation and test, considering whether the data had already split. We would separate 10\% of the training data for validation if the dataset did not have specific data for this measure. Table \ref{tab:datasets} shows the datasets used and how we split them for training, validation and testing for each model (Two-step or single-stage model). The first stage of the TS-UNETs had a total of 1169 training sampling, 484 validation sampling and 1775 test sampling. For the second and single-stage models, we obtained 1120 images for training, 479 for validation, and 1748 for testing. 


%For the multidataset, we took advantage of datasets that already had a predefined separation between training, validation, and testing (DRISHTI, REFUGE, and IDRID). With IDRID, the only drawback is that it has only disk masks, so it was used only for the first stage training. We also included the full RIGA dataset. There were 1253 images for the first stage training and 1199 images for the second stage training. For validation, 10\% of the training images were separated, except for REFUGE, which already had 400 images separated for this stage. Data sets from DRISHTI (test), REFUGE (test), RIMONE v3, ORIGA and PAPILA were used for the test stage.

%In this study, we based both model steps on the UNET architecture \cite{ronneberger2015unet}, designed for working on biomedical image segmentation. As we can see in the literature, this architecture is currently used in several problems, including OD/OC segmentation \cite{alawad2022machine}.

%UNET architecture consists of two parts, encoder and decoder. The encoder has four convolutional layers, which extract characteristics from the image and decrease dimensionality. On the other hand, the decoder has four up-sampling layers connected to a convolutional layer, which aims to return to the input resolution. In the centre, the bottleneck layer connects both structures. In addition, the encoder is connected to the decoder through skip connections, which allows recovering finer details of the prediction.

%We use outputs depths of 64, 128, 256, 512 and 1024 at each level for the encoder and the bottleneck layer. On the other hand, we utilize depths of 512, 256, 128 and 64 in the decoder layers. We apply a max-pooling of 2x2xdepth between each convolutional layer of the encoder. Each convolutional layer has 2 convolutional blocks which contain a convolutional filter (kernel=3, stride=1,padding=1), batch normalization and the rectified linear unit activation function (ReLU). On the other hand, the up-sampling layer with a factor of two is followed by two convolutional blocks, as mentioned above.

%La misma cuenta con ....... Codificador, decodificador, skip connections, cuántos canales, tamaño de kernel, stride, relu, softmax.... Batch size, numero de épocas, Learning rate. Adam. Reduce LR on plateau. Loss function. Data augmentation. 

%Both stages models' were trained in parallel. We applied the augmentation methods of Vertical Flip, Horizontal Flip, Gaussian Blur, Collor Jitter (brightness, contrast and saturation) and Random Affine (rotation and scaling). We were aiming for more generalization and avoiding overfitting. Augmentation methods were applied with different probability and strength, and we selected the set that resulted in a more accurate model. This augmentation selection was performed separately between stage 1 and stage 2.

%Both stages models' were trained in parallel. We applied the augmentation methods of Vertical Flip, Horizontal Flip, Gaussian Blur, Collor Jitter (brightness, contrast and saturation) and Random Affine (rotation and scaling). We were aiming for more generalization and avoiding overfitting. Augmentation methods were applied with different probability and strength, and we selected the set that resulted in a more accurate model. This augmentation selection was performed separately between stage 1 and stage 2.

%We use an Adam optimizer with an initial learning rate of 0.01 and a reduced lr on Plateau with a factor of 0.2 and patience of 2. We also employed a Cross-entropy as a loss function. We trained with a batch size of 5 for 200 epochs. In the case of training only with the DRISHTI dataset, we trained with 400 epochs due to the small amount of data in that set. We also used an early stopping technique to keep the model that gave us the best metric on the validation data.
 
 %For segmentation evaluation, we use the Dice coefficient, widely used in the literature like Wang et al. \cite{wang2019patch}, Shah et al.\cite{shah2019dynamic}, among others. With the Dice coefficient, we compare the similarity of the segmentation obtained by the model in contrast to the ground truth by calculating $Dice = (2* $Area of overlap)$/$ Total area. A Dice value closer to one implies that the model segmentation was similar to the ground truth.

%As mentioned in the Introduction, we need to calculate the vertical cup-to-disc ratio (vCDR) to detect glaucoma over fundus images. vCDR is calculated by computing the vertical distance of the cup and then dividing it by the vertical distance of the disc. $vCDR = dOC/dOD$. So a smaller vCDR value implies a larger difference between the distances of the optic disc and cup, which can be assumed to be a healthy subject. On the other hand, a larger vCDR value implies that the difference between the cup and disc distance is smaller, implying possible glaucoma.

%The receiver-operating characteristic (ROC) curve, which is very common in the literature, was used as a classification metric, in our case, between cases with or without glaucoma. The ROC curve is always accompanied by the value of the area under the curve (AUC), which indicates how well the glaucoma cases could be classified, in this case, calculated from the vCDR previously obtained. 




% \begin{figure}
%     \centering
%     \subcaptionbox{REFUGE}{
%     \includegraphics[width=0.18\textwidth]{Imgs/Fig5/Fig5a.pdf}}%
%     \hspace{0.01\textwidth}
%     \subcaptionbox{DRISHTI}{\includegraphics[width=0.18\textwidth]{Imgs/Fig5/Fig5b.pdf}}%
%     \hspace{0.01\textwidth}
%     \subcaptionbox{RIM ONE v3}{\includegraphics[width=0.18\textwidth]{Imgs/Fig5/Fig5c.pdf}}%
%     \hspace{0.01\textwidth}
%     \subcaptionbox{ORIGA}{\includegraphics[width=0.18\textwidth]{Imgs/Fig5/Fig5d.pdf}}%
%     \hspace{0.01\textwidth}
%     \subcaptionbox{PAPILA}{\includegraphics[width=0.18\textwidth]{Imgs/Fig5/Fig5e.pdf}}%
%   \caption{Scatter plots comparing the vertical cup-to-disc ratio (vCDR) estimated from our predicted segmentation and from the ground truth annotations in (a) DRISHTI, (b) REFUGE, (c) RIM ONE v3, (d) ORIGA y (e) PAPILA}
%     \label{fig:vcdr}
% \end{figure}


% \begin{figure}
%     \centering
%     \subcaptionbox{REFUGE}{\includegraphics[width=0.19\textwidth]{Imgs/Fig6/REFUGE_ROC_glaucoma.pdf}}%
%     \hspace{0.001\textwidth}
%     \subcaptionbox{DRISHTI}
%     {\includegraphics[width=0.19\textwidth]{Imgs/Fig6/DRISHTI_ROC_glaucoma.pdf}}%
%     \hspace{0.001\textwidth}
%     \subcaptionbox{RIMONE v3}
%     {\includegraphics[width=0.19\textwidth]{Imgs/Fig6/rimone_ROC_glaucoma.pdf}}%
%     \hspace{0.001\textwidth}
%     \subcaptionbox{ORIGA}
%     {\includegraphics[width=0.19\textwidth]{Imgs/Fig6/origa_ROC_glaucoma.pdf}}%
%     \hspace{0.001\textwidth}
%     \subcaptionbox{PAPILA}
%     {\includegraphics[width=0.19\textwidth]{Imgs/Fig6/Papila_ROC_glaucoma.pdf}}%

%     \caption{Glaucoma assessment results obtained in (a) DRISHTI, (b) REFUGE, (c) RIM ONE v3, (d) ORIGA, (d) PAPILA. Left: ROC curves obtained for glaucoma detection using the vertical cup-to-disc ratio (vCDR) estimated from our automated segmentation. The result obtained by SS-MODEL is marked in grey. Results obtained by the TS-MODEL is marked in blue, and results obtained by the ground truth segmentation are marked in pink}
%     \label{fig:roc-curves}
% \end{figure}


% FIGURA PAPILA (NO LA VAMOS A PONER)
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Imgs/Fig4.pdf}
%     \caption{Good (left), median (center) and bad (right) qualitative results obtained in the PAPILA dataset with the TS-MODEL $OD \rightarrow OD & OC$}
%     \label{fig:qualitative-papila}
% \end{figure}






% Tabassum \textit{\textit{et al}.} \cite{tabassum2020cded} introduces a novel architecture specifically crafted for computational efficiency during training.
% It trains on each specific dataset, using 70\% for training and 30\% for test. The models are then super specialized to each set!
    % SS and TS models perform better for OD segmentation when trained on DRISHTI and the multi-dataset, while being almost equivalent when trained using REFUGE data.
    % OC segmentation results in DRISHTI are comparable when SS and TS are trained in the combined dataset, but remain lower when trained on DRISHTI and REFUGE.
    % In RIM-ONE v3, Tabassum \textit{\textit{et al}.} \cite{tabassum2020cded} reported higher Dice values for both OD/OC segmentation. This could be because they used images from RIM-ONE v3 for training. In our case, we saved it as a test set.




% Al-Bandet
Al-Bandet \textit{\textit{et al}.} \cite{al2018dense}, for instance, uses a combination of a U-shaped fully convolutional DenseNet and a postprocessing strategy to segment images that are manually cropped and rescaled. Hence, this method could be seen as a two-stage approach in which the first part is handled by the user. Their results in ORIGA are much higher than ours for OD segmentation, although it should be pointed out that their model was trained on 70\% of the ORIGA data and evaluated in the remaining 30\%. On the contrary, our two models were trained on separate databases and evaluated on the entire ORIGA set, and achieved much higher Dice values for OC segmentation.
% Shah
Shah \textit{et al.} \cite{shah2019dynamic} also achieved a better average Dice for OD segmentation than ours, in this case in RIM-ONE v3. Their model consists of a coarse-to-fine approach similar to our TS (OD - OD \& OC), although both stages share the same encoder and are trained in an end-to-end manner. Similar to what we observed before, they trained and evaluated their method in subsets of RIM ONE v3, while we used all RIM ONE images for testing.


\cite{al2018dense,liu2021joint}


% Al-Bander
Al-Bandet \textit{\textit{et al}.} \cite{al2018dense}, for instance, uses a combination of a U-shaped fully convolutional DenseNet and a postprocessing strategy to segment images that are manually cropped and rescaled. Hence, this method could be seen as a two-stage approach in which the first part is handled by the user. Our models, on the contrary, perform directly on the input image without requiring any manual intervention, and achieve much better results in almost all scenarios. Their approach only outperforms ours for OD segmentation in ORIGA, although it should be pointed out that it was trained on 70\% of the ORIGA data and evaluated in the remaining 30\%. On the contrary, our two models were trained on separate databases and evaluated on the entire ORIGA set.
% Team BUCT
Team BUCT originally ranked third in REFUGE \cite{orlando2020refuge} using two separate U-Nets, one for each class. Their OD network takes input images cropped around the FOV as input, and the OC one is applied on crops around the OD prediction. This setting is similar to our TS (OD - OC) model, as no OD supervision is used in the OC segmentation part. As their models were trained only with REFUGE data, the most fair comparison is using SS and TS indicated as (REFUGE) in Table \ref{tab:dice}, which achieved better average Dice values for OD/OC segmentation.
% 



% Wang \textit{\textit{et al}.} \cite{wang2019patch}. Coarse to fine similar to the TS (OD - OD & OC) but using an adversarial loss with a patch-based discriminator, a shape-aware objective and a domain adaptation strategy. This combination of techniques was designed to improve results when applied on previously unseen datasets.
% They train their model in REFUGE and evaluated it in REFUGE, DRISHTI, RIM-ONE v3
    % Using the same setting:
        % SS and TS models performed better in REFUGE for OD segmentation. For OC segmentation, SS reported results 4% higher, while TS results are almost equivalent.
        % When evaluated in DRISHTI, both SS and TS obtained almost identical average Dice values for the OD, while OC results are superior.
        % In RIM ONE v3, Wang \textit{et al}. obtained the best results for both classes.
% Nevertheless, both SS and TS trained on the multi-dataset configuration achieved better results in all databases both for OD/OC segmentation, meaning that domain adaptation might not be necessary if enough training data is available.

% Shah \textit{\textit{et al}} \cite{shah2019dynamic} is also a coarse-to-fine network similar to TS (OD - OD & OC) although the second network uses the pre-trained weights of the encoder of the first network. Furthermore, the entire model is trained in an end-to-end manner instead of separately.
% They train their model using DRISHTI images and a subset of RIM ONE v3, separately.
    % In DRISHTI, both our SS and TS models achieved slightly better results for OD/OC segmentation when trained on DRISHTI.
    % In RIM ONE v3, both approaches reported less accurate performance for OD segmentation even trained on a multi-dataset setting, while being almost equivalent for OC segmentation. 




    
% Liu \textit{\textit{et al}.} \cite{liu2021joint} is similar than our TS (OD - OD & OC) model. Changes in network design.
% Model evaluated in REFUGE was trained in REFUGE
    % SS and TS achieved better OD results when trained and evaluated using the same data.
    % SS obtained higher OC results, while TS is almost equal.
% Model evaluated in DRISHTI was trained in DRISHTI
    % Liu model outperforms ours in both tasks yet average Dice is quite similar.
% If SS and TS models are trained with the combined dataset, both perform similarly to it or even better, despite the fact it does not incorporates any network innovation.
    

    

% TEXTO TUYO ANTERIOR:
%Table \ref{tab:dice} shows the Dice obtained for OD/OC segmentation, both the TS-MODEL ($OD \rightarrow OD \& OC$) and the SS-MODEL trained with DRISHTI, REFUGE and multi-dataset training set. Also,  different models present in the literature are presented in the Table.
%
%In the models trained with DRISHTI, we can observe better OD/OC segmentation with the TS-MODEL, except for the segmentation on RIM ONE v3. On the other hand, in the models trained with REFUGE data, the results are more varied. TS-MODEL obtained better results for OD segmentation on the REFUGE and DRISHTI test data. In contrast, the SS-MODEL obtained better OD segmentations for the RIM ONE v3 and ORIGA datasets. For OC segmentation, the model trained with the two-stage REFUGE obtained better results in segmenting the DRISHTI data, while SS-MODEL obtained better results in the rest of the datasets.
%
%We compare the models trained with DRISHTI to those trained with REFUGE. We observe that, in general, the model trained with REFUGE obtains better results for both disc and cup segmentation. However, this does not occur when the model has to segment the DRISHTI test data where the model trained with DRISHTI obtained better results. 
%
%The models trained with multiple datasets performed better than their counterparts trained on a single dataset. Both the TS-MODEL and the SS-MODEL obtained generally similar values. TS-MODEL obtained better values for the ORIGA dataset, while SS-MODEL obtained a higher Dice for the RIM ONE dataset [for discussion: Does the training data matter more?]
%
%Compared with literature approaches, our models obtain better or equal values. For REFUGE segmentation, our SS-MODEL and TS-MODEL obtained better results in OD than those presented in the literature. While for OC segmentation, the SS-MODEL was the one with better results. On DRISHTI data, a better result is observed in the work of Liu \textit{et al}.\cite{liu2021joint} for the OD and Tabassum \textit{et al}.\cite{tabassum2020cded} for the OC but always followed by our models. A significant difference is observed in the RIM ONE v3 segmentation, where Tabassum \textit{et al}. approac obtained better results for OD/OC. Finally, for the ORIGA dataset, a similar result is observed between our TS-MODEL and the work of Al-Bandet \textit{et al}.\cite{al2018dense} for OD segmentation. At the same time, the TS-MODEL model obtained the best results for the OC. 






% TEXTO TUYO ANTERIOR
%Figures \ref{fig:qualitative-all} and \ref{fig:qualitative-papilla} show qualitative examples of OD/OC segmentation obtained with the TS-MODEL $OD \rightarrow OD & OC$ over various test data. Three examples of each dataset are shown in the figures, a good, an average and a bad segmentation. In addition to the segmentation, the figure shows the original image, cut in the OD region, and their ground truth.
%
%We can observe that each model can distinguish the OD and OC from the rest of the image, even in the worst case. Even with a significant difference in colour and contrast between the different data sets.
%
%For the segmentation of the REFUGE data, the model had results almost identical to the ground truth. The same happens when segmenting DRISHTI data. In the case of the RIM ONE v3 data, we observe differences between the segmentation and the ground truth. The obtained result stops having an ellipse shape, especially in the average and bad samples. For the ORIGA dataset, a closer approximation to ground truth is obtained with more accurate segmentation. Only in the lousy segmentation sample is an open OD area observed. Finally, for the PAPILA dataset, an OD deformation is observed in one of the samples. At the same time. A remarkable difference was obtained in the OC in those segmentations where a more rounded segmentation was obtained, Where a large OC was segmented compared to the ground truth.





%vCDR
Subsequently, we analyzed whether we can use our segmentation model as an early detector of signs of possible glaucoma. For this purpose, we calculate the vertical cup-to-disc ratio (vCDR). We estimate this metric for the segmentation obtained by TS-MODEL ($OD \rightarrow OD \& OC$) and the segmentation given as ground truth. The vCDR ratio was also examined in both healthy and glaucoma cases.


Figure \ref{fig:vcdr} shows the relationship between the vCDR calculated from our segmentation compared to the vCDR obtained from the ground truth. The best results are observed with the REFUGE and DRISHTI datasets, with a Pearson Coefficient of 0.75 and 0.87, respectively. [discussion. These datasets were previously observed by the model with its 3 datasets. followed by the results of RIM ONE (r= 0.54), ORIGA (r= 0.35) and finally the results of PAPILA (r= 0.25). 




Figure \ref{fig:roc-curves} shows the ROC curve obtained from the vCDR, calculated on the segmentations, for glaucoma classification. We compare the resulting values from the TS-MODEL ($OD \rightarrow OD \& OC$) and the SS-MODEL. Both showed an AUC above 70\%, but we obtained an AUC of 60\% for the suspect cases over the PAPILA dataset. 

In the REFUGE classification, it can be observed that the SS-MODEL model was the one that gave the best results, being even better than the one obtained from the ground truth segmentation. For the classification of the DRISHTI data, we appreciate that the TS-MODEL is the one that obtained the betters results. However, the classification of both models is below the one obtained by the ground truth. For the RIM ONE data, similar results are observed for the TS-MODEL, the SS-Model and the one obtained by the Ground truth. For ORIGA, we notice that TS-MODEL obtained a much better glaucoma classification than SS-Model and the one obtained from the ground truth. Finally, for the PAPILA data, we see that the TS-Model obtained a better classification than the SS-Model, although below the ground truth for both models. The same happened for the classification of glaucoma cases and suspected glaucoma cases.


Figure \ref{fig:vcdr_airogs} shows the results of comparing the vCDR obtained from the model segmentation (TS-UNET $OD \rightarrow OD \& OC$) and the vCDR given by six experts. In box-plot (a), we can observe that for glaucoma cases, the model obtained similar vCDR's to the one generated by experts. While in non-glaucoma cases, we can appreciate a significant difference concerning the experts. In glaucoma cases, we observe that a couple of experts differ from the rest. While for the cases without glaucoma, we can observe more similar results except for the last two experts.

On the other hand, the graph in Figure \ref{fig:vcdr_airogs} (b) shows the roc curve obtained by all the experts and the TS-MODEL from the calculated vCDR. We can appreciate a similarity between the results obtained with the model and those obtained by the experts. We can appreciate the similarity in the curve obtained and in the AUC resulting.
